What If Moderation Didn't Mean Suppression? A Case for Personalized Content Transformation

Centralized content moderation paradigm both falls short and over-reaches: 1) it fails to account for the subjective nature of harm, and 2) it acts with blunt suppression in response to content deemed harmful, even when such content can be salvaged. We first investigate this through formative interviews, documenting how seemingly benign content becomes harmful due to individual life experiences. Based on these insights, we developed DIY-MOD, a browser extension that operationalizes a new paradigm: personalized content transformation. Operating on a user's own definition of harm, DIY-MOD transforms sensitive elements within content in real-time instead of suppressing the content itself. The system selects the most appropriate transformation for a piece of content from a diverse palette--from obfuscation to artistic stylizing--to match the user's specific needs while preserving the content's informational value. Our two user studies demonstrate that this approach increases users' sense of agency and safety, enabling them to engage with content and communities they previously needed to avoid.

==> abstract.tex <==
%%%% (150 words below. Limit 150)

% We argue that the current paradigm of centralized content moderation both falls short and overreaches: 1) It cannot account for the highly personal, situational nature of harm, and 2) it acts with blunt suppression in response to contents deemed harmful, even when such content can be salvaged so that the user may still engage with its valuable parts. We shed light on these problems through interviews with people revealing accounts of content that, while mundane or even benign to most, becomes harmful in light of a person's particular history or circumstances. These cases highlight how individuals are often forced to navigate a trade-off between maintaining their well-being and staying engaged in online spaces. We use these accounts as a starting point for designing a browser extension, \diymod{}, that lets end users moderate such content themselves. Instead of defining harm universally or relying on content removal, we operationalize \emph{personalized content transformation} as a new paradigm for moderation. We define a design space of possible transformations, which \diymod{} selects from in real-time based on what it knows about the user, aiming to mitigate elements they perceive as harmful while preserving the content's informational or social value. Through a user study with users using \diymod{} on their Reddit Feeds, we learn...



Centralized content moderation paradigm both falls short and overreaches: 1) it fails to account for the subjective nature of harm, and 2) it acts with blunt suppression in response to content deemed harmful, even when such content can be salvaged. We first investigate this through formative interviews, documenting how seemingly benign content becomes harmful due to individual life experiences. Based on these insights, we developed \diymod{}, a browser extension that operationalizes a new paradigm: \emph{personalized content transformation}. Operating on a user's own definition of harm, \diymod{} transforms sensitive elements within content in real-time instead of suppressing the content itself. The system selects the most appropriate transformation for a piece of content from a diverse palette---from obfuscation to artistic stylizing---to match the user's specific needs while preserving the content's informational value. Our two-session user study demonstrates that this approach increases users' sense of agency and safety, enabling them to engage with content and communities they previously needed to avoid.


==> selection_3.tex <==


The core of DIY-MOD is a policy model, the `Selector', which learns to choose an appropriate intervention $I$ from our palette $\mathcal{I}$ for a given context $C$. We emphasize that content moderation involves navigating trade-offs rather than finding singular correct answers---multiple interventions may effectively serve a user's needs with different characteristics. Our approach demonstrates one viable method for learning these trade-offs through a combination of expert knowledge, automated evaluation, and user preferences.



The context vector $C = [c_{sens}, c_{sal}, c_{scale}, c_{feas}, c_{mod}]$ captures user preferences and content properties as detailed in our framework design (Section \ref{section:framework}). The `Selector', implemented as a gradient boosting classifier (XGBoost), learns to map this context vector to suitable interventions through our three-phase training process.

\subsection{Phase 1: Establishing Baseline Model}

We initialize the `Selector' through supervised learning on an expert-curated dataset $\mathcal{D}_{SFT} = \{(C_i, I_i^*)\}_{i=1}^N$, where $I_i^*$ represents the intervention deemed most appropriate by the research team \rayhan{We label and combine} for context $C_i$. This phase provides a sensible starting policy grounded in domain expertise, though we acknowledge these labels represent one reasonable approach among many valid alternatives.

\subsection{Phase 2: Learning Relative Preferences}

To refine our baseline model beyond individual expert judgments, we generate a larger dataset capturing relative intervention quality. This automated process enables the model to learn nuanced trade-offs between different approaches.

\subsubsection{Multi-Criteria Evaluation Framework}

We employ an LLM-based `Rubric Judge' to evaluate intervention outcomes along the three dimensions established in our framework: Goal Alignment ($s_{goal}$), Resulting Coherence ($s_{coh}$), and Factual Integrity ($s_{fact}$). These dimensions, grounded in prior work on factual consistency \cite{ji2022survey}, content coherence \cite{fabbri2021summeval}, and goal-directed evaluation \cite{basili1994gqm}, enable systematic comparison of intervention quality.



% We employ an LLM-based `Rubric Judge' to evaluate intervention outcomes along three key dimensions:

% \begin{itemize}
%     \item \textbf{Goal Alignment ($s_{goal}$):} Measures how effectively the intervention achieves its intended purpose---reducing exposure to triggering content while preserving user agency.
    
%     \item \textbf{Resulting Coherence ($s_{coh}$):} Assesses output quality---whether modified content remains plausible, logical, and visually/textually natural.
    
%     \item \textbf{Factual Integrity ($s_{fact}$):} Evaluates whether objective, verifiable facts are preserved, serving as a guardrail against misinformation.
% \end{itemize}

\subsubsection{Generating Preference Data}

We convert multi-criteria evaluations into preference pairs using a utility function:
\begin{equation}
    U(S) = w_{goal} \cdot s_{goal} + w_{coh} \cdot s_{coh} + w_{fact} \cdot s_{fact}
\end{equation}

Our weights ($w_{goal}=2.0$, $w_{coh}=1.0$, $w_{fact}=0.5$) reflect prioritizing functional effectiveness and output quality---a design choice that emphasizes user protection while maintaining content intelligibility. Algorithm \ref{alg:pref_gen} details our preference generation process.

\begin{algorithm}[H]
\caption{Automated Preference Pair Generation}
\label{alg:pref_gen}
\begin{algorithmic}[1]
\Require Expert dataset $\mathcal{D}_{SFT}$, Intervention palette $\mathcal{I}$, Utility function $U$
\Ensure Preference dataset $\mathcal{D}_{AP}$
\State $\mathcal{D}_{AP} \gets \emptyset$
\For{each $(C_i, I_i^*) \in \mathcal{D}_{SFT}$}
    \For{each alternative $I_{alt} \in \mathcal{I} \setminus \{I_i^*\}$} \Comment{Compare against all alternatives}
        \State $S_i^* \gets \Call{RubricJudge}{C_i, I_i^*}$
        \State $S_{alt} \gets \Call{RubricJudge}{C_i, I_{alt}}$
        \State $\Delta U \gets U(S_i^*) - U(S_{alt})$
        \If{$|\Delta U| > \epsilon$} \Comment{Skip near-ties}
            \State Add $(C_i, I_{winner}, I_{loser})$ to $\mathcal{D}_{AP}$ with margin $|\Delta U|$
        \EndIf
    \EndFor
\EndFor
\State \Return $\mathcal{D}_{AP}$
\end{algorithmic}
\end{algorithm}

\subsubsection{Preference-Aware Training}

We transform preference data into weighted training samples for XGBoost refinement. For each preference tuple $(C, I_w, I_l, \Delta U) \in \mathcal{D}_{AP}$, we construct a weighted training dataset $\mathcal{D}_{train}^{(2)}$ as follows:

\begin{equation}
\mathcal{D}_{train}^{(2)} = \bigcup_{(C, I_w, I_l, \Delta U) \in \mathcal{D}_{AP}} \left\{ (C, I_w, w^+), (C, I_l, w^-(\Delta U)) \right\}
\end{equation}

where the sample weights are defined as:
\begin{align}
w^+ &= 1.0 \\
w^- &= \max(0.1, 1.0 - \Delta U)
\end{align}

This weighting scheme serves two purposes: it reinforces the model's preference for superior interventions while maintaining learning signal from inferior options, particularly when margins are small. Close comparisons ($\Delta U \approx 0$) receive nearly equal weights, preserving crucial information about decision boundaries. The XGBoost model update is then:

\begin{equation}
\theta^{(2)} = \arg\min_{\theta} \sum_{(C_j, I_j, w_j) \in \mathcal{D}_{train}^{(2)}} w_j \cdot \mathcal{L}(f_{\theta}(C_j), I_j)
\end{equation}

where $\mathcal{L}$ is the multi-class logarithmic loss and $f_{\theta}$ represents the XGBoost model with parameters $\theta$.

\subsection{Phase 3: Human Preference Alignment}

While automated evaluation provides scalable training signals, genuine user preferences capture subtleties that programmatic metrics cannot fully represent. This phase represents a critical departure from purely algorithmic optimization toward genuine user-centered design.

\subsubsection{Preference Elicitation Protocol}

We collect human preferences through a carefully designed user study protocol. Participants interact with DIY-MOD in real-world browsing scenarios and periodically encounter preference elicitation interfaces. For a given context $C_k$, we present two intervention outcomes side-by-side---for instance, the same triggering image processed through `Blur' versus `Stylize'. Participants select their preferred outcome based on their personal comfort and information needs.

This process generates dataset $\mathcal{D}_{HP} = \{(C_k, I_{chosen}^k, I_{rejected}^k)\}_{k=1}^M$, where each entry represents a genuine user preference in a specific context. Importantly, we collect preferences across diverse contexts to capture the full range of user needs---from situations where complete occlusion is desired to cases where subtle modification suffices.

\subsubsection{Incorporating Human Judgments}

Human preferences often reveal patterns that diverge from our utility function's predictions. A user might prefer `Stylize' over `Inpainting' despite the latter scoring higher on goal alignment, perhaps valuing the artistic transformation's psychological distance from the trigger. We honor these preferences by constructing a final training dataset:

\begin{equation}
\mathcal{D}_{train}^{(3)} = \bigcup_{(C_k, I_{chosen}^k, I_{rejected}^k) \in \mathcal{D}_{HP}} \left\{ (C_k, I_{chosen}^k, w_{human}^+), (C_k, I_{rejected}^k, w_{human}^-) \right\}
\end{equation}

We employ stronger weight differentiation for human preferences ($w_{human}^+ = 1.0$, $w_{human}^- = 0.1$) to ensure these genuine user signals effectively override automated preferences where conflicts exist. The final model parameters are:

\begin{equation}
\theta^{(3)} = \arg\min_{\theta} \sum_{(C_j, I_j, w_j) \in \mathcal{D}_{train}^{(3)}} w_j \cdot \mathcal{L}(f_{\theta^{(2)}}(C_j), I_j)
\end{equation}

where we initialize from $\theta^{(2)}$ to preserve learned patterns while adapting to human preferences.


\subsubsection*{Summary: }This three-phase training pipeline—expert initialization, automated preference learning, and human alignment—enables DIY-MOD to learn nuanced intervention selection while remaining computationally efficient for real-time deployment. By combining multiple sources of knowledge in a structured progression, we demonstrate that effective personalized content moderation can emerge from relatively simple components when properly orchestrated. The resulting `Selector' model provides context-aware intervention selection that balances user protection with information preservation, as we evaluate in the following section.
